Towards Secure and Usable 3D Assets: A Novel Framework for Automatic Visible Watermarking

3D models, particularly AI-generated ones, have witnessed a recent surge across various industries such as entertainment. Hence, there is an alarming need to protect the intellectual property and avoid the misuse of these valuable assets. As a viable solution to address these concerns, we rigorously define the novel task of automated 3D visible watermarking in terms of two competing aspects: watermark quality and asset utility. Moreover, we propose a method of embedding visible watermarks that automatically determines the right location, orientation, and number of watermarks to be placed on arbitrary 3D assets for high watermark quality and asset utility. Our method is based on a novel rigid-body optimization that uses back-propagation to automatically learn transforms for ideal watermark placement. In addition, we propose a novel curvature-matching method for fusing the watermark into the 3D model that further improves readability and security. Finally, we provide a detailed experimental analysis on two benchmark 3D datasets validating the superior performance of our approach in comparison to baselines. Code and demo are available.

==> sections/todo.tex <==
\section{Todo}

\begin{enumerate}
    \item Include results of meshy dataset inside the main body. (\cindy{Cindy - done, see \cref{tab:results}} )
    \item Try to fit Table 1 into one column (Cindy).
    \item Change Figure 3 to include better and more qualitative results. Use zoom functionality. Make it fit into one column (Cindy).
    \item Change Figure 2 to fit into one column. (Cindy)
    \item Add attack results from the paper (table and qual pictures) (\cindy{Cindy - done, see \cref{sec:attacks}}).
    \item Review and proof read the prob def. section. (Simar)
    \item Make concise - method: candidate generation, filtering and embossing (Simar)
    \item Make concise - experiments: evaluation metrics (Simar)
    
\end{enumerate}
